FaceMAE: Privacy-Preserving Face Recognition via Masked Autoencoders

Face recognition, as one of the most successful applications in artificial intelligence, has been widely used in security, administration, advertising, and healthcare. However, the privacy issues of public face datasets have attracted increasing attention in recent years. Previous works simply mask most areas of faces or synthesize samples using generative models to construct privacy-preserving face datasets, which overlooks the trade-off between privacy protection and data utility. In this paper, we propose a novel framework FaceMAE, where the face privacy and recognition performance are considered simultaneously. Firstly, randomly masked face images are used to train the reconstruction module in FaceMAE. We tailor the instance relation matching (IRM) module to minimize the distribution gap between real faces and FaceMAE reconstructed ones. During the deployment phase, we use trained FaceMAE to reconstruct images from masked faces of unseen identities without extra training. The risk of privacy leakage is measured based on face retrieval between reconstructed and original datasets. Experiments prove that the identities of reconstructed images are difficult to be retrieved. We also perform sufficient privacy-preserving face recognition on several public face datasets (i.e. CASIA-WebFace and WebFace260M). Compared to previous state of the arts, FaceMAE consistently \textbf{reduces at least 50\% error rate} on LFW, CFP-FP and AgeDB.

==> author.tex <==
\author{
Kai Wang\textsuperscript{1}\thanks{Equal contribution. (kai.wang@comp.nus.edu.sg, bo.zhao@ed.ac.uk)} 
\quad Bo Zhao\textsuperscript{2}\footnotemark[1]
\quad Xiangyu Peng\textsuperscript{1}
\quad Zheng Zhu\textsuperscript{3}
\quad Shuo Yang\textsuperscript{4}
\quad Shuo Wang\textsuperscript{5}
\\
\quad Guan Huang \textsuperscript{3}
\quad Hakan Bilen\textsuperscript{2}
\quad Xinchao Wang \textsuperscript{1}
\quad Yang You\textsuperscript{1}\thanks{Corresponding author (youy@comp.nus.edu.sg).}
% \quad Yichen Zhou\textsuperscript{1, 2}
% \\
% \quad Xinchao Wang\textsuperscript{2}
% \quad Jiashi Feng\textsuperscript{1}
% \quad Shuicheng Yan\textsuperscript{1}
\\
\textsuperscript{1}{National University of Singapore}
\quad \textsuperscript{2}{The University of Edinburgh}
\quad \textsuperscript{3}{PhiGent Robotics}
\\
\quad \textsuperscript{4}{University of Technology Sydney}
\quad \textsuperscript{5}{Institute of Automation, Chinese Academy of Sciences}

% \\
% \small{\texttt{\{xiangyupeng, kai.wang, youy\}@comp.nus.edu.sg} \quad \texttt{zhengzhu@ieee.org}}
\\
\small{Code: \url{https://github.com/kaiwang960112/CAFE}}
}

==> table/abl.tex <==
\begin{table}[h]
% \begin{minipage}{0.525\linewidth}
    \centering
    \begin{tabular}{ccc|ccc}
    \toprule
     \multicolumn{3}{c}{Operation} & \multicolumn{3}{|c}{Evaluation Datasets}\\
			\cmidrule{1-6}
			 Pretrain on ImageNet & Intance Matching &Relation Matching & LFW & CFP-FP &AgeDB\\
			\midrule
			&&&&&\\
			&\checkmark&&98.30&86.2&86.1\\
			&&\checkmark&&&\\
			&\checkmark&\checkmark&&&\\
			\checkmark &&&&&\\
			\checkmark &\checkmark&&98.83&89.17&90.18\\
			\checkmark &&\checkmark&98.16&83.58&84.63\\
			\checkmark &\checkmark&\checkmark&&&\\
			
			\bottomrule
			
        %  Pretrain & IM &IRM & CIFAR-10 & CIFAR-100\\
        %  \hline
        %  && 83.9 & 31.5\\
        %  \checkmark & &85.3 & 36.3\\
        %  & \checkmark &89.8 & 41.8 \\
        %  \checkmark &\checkmark &\textbf{93.5}&\textbf{48.4} \\
    \end{tabular}
    \caption{Evaluation of ReCo and H-Aug. in the proposed framework. The noise type is 90\% symmetric noise for both CIFAR-10 and CIFAR-100. \textbf{Bold entries} are best results.}
    \label{tab:abl_module}
\end{table}

% \end{minipage}


% \hspace{5mm}\begin{minipage}{0.425\linewidth}
%     \centering
%     \begin{tabular}{c|c|c|c}
%          ReCo & H-Aug. & CIFAR-10 & CIFAR-100\\
%          \hline
%          && 83.9 & 31.5\\
%          \checkmark & &85.3 & 36.3\\
%          & \checkmark &89.8 & 41.8 \\
%          \checkmark &\checkmark &\textbf{93.5}&\textbf{48.4} \\
%     \end{tabular}
%     \caption{Evaluation of ReCo and H-Aug. in the proposed framework. The noise type is 90\% symmetric noise for both CIFAR-10 and CIFAR-100. \textbf{Bold entries} are best results.}
%     \label{tab:hhh}
% \end{minipage}
% \end{table}

==> table/abl_v2.tex <==
\begin{table}[h]
\begin{minipage}{0.32\linewidth}
    \centering
    \small
    \resizebox{\linewidth}{0.24\linewidth}{
    \begin{tabular}{ccc|ccc}
    \toprule
    
%     \multicolumn{2}{c}{Operation} & \multicolumn{3}{|c}{Evaluation Datasets}\\
% 			\cmidrule{1-5}
% 			 $\mathbf{L_{mse}}$ & IRM & LFW & CFP-FP &AgeDB\\
% 			\midrule
% 			&&97.62&87.14&85.68 \\
% 			\checkmark &&98.23&87.29&86.17\\
% 			&\checkmark &&&\\
% 			\checkmark &\checkmark &98.93&90.80&90.18\\
% 			\bottomrule
% 			 \end{tabular}}
    
    %########## IM RM#########
     \multicolumn{3}{c}{Operation} & \multicolumn{3}{|c}{Evaluation Datasets}\\
			\cmidrule{1-6}
			 $\mathbf{L_{mse}}$ & IM &RM & LFW & CFP-FP &AgeDB\\
			\midrule
			&&&97.62&87.14&85.68 \\
			\checkmark &&&98.23&87.29&86.17\\
% 			&\checkmark &&&&\\
% 			&&\checkmark &&&\\
			\checkmark &\checkmark &&98.93&89.69&89.78\\
			\checkmark &&\checkmark &98.92&87.10&86.68\\
			\checkmark &\checkmark&\checkmark &\textbf{99.23}&\textbf{90.80}&\textbf{90.25}\\
				\bottomrule
			 \end{tabular}}
%############################################################
   \vspace{0.2em}
    \caption{Evaluation of $\mathbf{L_{mse}}$, IM and RM in the proposed \textit{FaceMAE}. \textbf{Bold entries} are best results.}
    \label{tab:mask_ratio}


\end{minipage}\hspace{3mm}\begin{minipage}{0.32\linewidth}
    \centering
    \small
    \resizebox{\linewidth}{0.24\linewidth}{
    \begin{tabular}{c|ccccc}
    \toprule
     \multirow{2}{*}{Mask Ratio} & \multicolumn{3}{|c}{Evaluation Datasets}\\
			\cmidrule{2-4}
			  & LFW & CFP-FP &AgeDB\\
			\midrule
			0.3&99.41&93.03&92.87\\
			0.5&99.33&91.98&91.56\\
			0.75&99.23&90.80&90.25\\
			0.9&67.33&57.38&54.01\\
% 			&&&&&\\
% 			&\checkmark&&98.30&86.2&86.1\\
% 			&&\checkmark&&&\\
% 			&\checkmark&\checkmark&&&\\
% 			\checkmark &&&&&\\
% 			\checkmark &\checkmark&&98.83&89.17&90.18\\
% 			\checkmark &&\checkmark&98.16&83.58&84.63\\
% 			\checkmark &\checkmark&\checkmark&&&\\
			
			\bottomrule
			
        %  Pretrain & IM &IRM & CIFAR-10 & CIFAR-100\\
        %  \hline
        %  && 83.9 & 31.5\\
        %  \checkmark & &85.3 & 36.3\\
        %  & \checkmark &89.8 & 41.8 \\
        %  \checkmark &\checkmark &\textbf{93.5}&\textbf{48.4} \\
    \end{tabular}}
     \vspace{0.2em}
    \caption{Evaluation of mask ratio of input faces for \textit{FaceMAE} training. All the mask patches are generated by random seed.}
    \label{tab:abl_module}

\end{minipage}\hspace{3mm}\begin{minipage}{0.32\linewidth}
    \centering
    \small
    \resizebox{\linewidth}{0.24\linewidth}{
    \begin{tabular}{c|c|cccc}
    \toprule
     \multirow{2}{*}{Train} & \multirow{2}{*}{Deploy} & \multicolumn{3}{c}{Evaluation Datasets}\\
			\cmidrule{3-5}
			 && LFW & CFP-FP &AgeDB\\
			\midrule
			
			W. & C. &99.23&90.80&90.25\\
% 			C. & C. &98.83&90.47&90.15\\
			C. & W. &99.37&93.87&94.14\\
			W.$_{sub1}$ & W.$_{sub2}$ &99.65&94.00&94.36\\
			W.$_{sub2}$ & W.$_{sub1}$ &99.47&94.12&94.51\\
% 			WebFace260m & CASIA-WebFace &&&\\
% 			CASIA-WebFace & CASIA-WebFace &&&\\
% 			CASIA-WebFace & WebFace260m &&&\\
			
% 			&&&&&\\
% 			&\checkmark&&98.30&86.2&86.1\\
% 			&&\checkmark&&&\\
% 			&\checkmark&\checkmark&&&\\
% 			\checkmark &&&&&\\
% 			\checkmark &\checkmark&&98.83&89.17&90.18\\
% 			\checkmark &&\checkmark&98.16&83.58&84.63\\
% 			\checkmark &\checkmark&\checkmark&&&\\
			
			\bottomrule
			
        %  Pretrain & IM &IRM & CIFAR-10 & CIFAR-100\\
        %  \hline
        %  && 83.9 & 31.5\\
        %  \checkmark & &85.3 & 36.3\\
        %  & \checkmark &89.8 & 41.8 \\
        %  \checkmark &\checkmark &\textbf{93.5}&\textbf{48.4} \\
    \end{tabular}}
     \vspace{0.2em}
    \caption{Evaluation of the generalization of \textit{FaceMAE}. W. and C. represent WebFace260m and CASIA-WebFace.}
    \label{tab:cross_dataset}


\end{minipage}
\end{table}


%\begin{minipage}{0.425\linewidth}
%     \centering
%     \begin{tabular}{c|c|c|c}
%          ReCo & H-Aug. & CIFAR-10 & CIFAR-100\\
%          \hline
%          && 83.9 & 31.5\\
%          \checkmark & &85.3 & 36.3\\
%          & \checkmark &89.8 & 41.8 \\
%          \checkmark &\checkmark &\textbf{93.5}&\textbf{48.4} \\
%     \end{tabular}
%     \caption{Evaluation of ReCo and H-Aug. in the proposed framework. The noise type is 90\% symmetric noise for both CIFAR-10 and CIFAR-100. \textbf{Bold entries} are best results.}
%     \label{tab:hhh}
% \end{minipage}
% \end{table}

==> tex/check_list.tex <==
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
